Quadratic Modelings of Syndrome Decoding

This paper presents enhanced reductions of the bounded-weight and exact-weight Syndrome Decoding Problem (SDP) to a system of quadratic equations. Over $\mathbb{F}_2$, we improve on a previous work and study the degree of regularity of the modeling of the exact weight SDP. Additionally, we introduce a novel technique that transforms SDP instances over $\mathbb{F}_q$ into systems of polynomial equations and thoroughly investigate the dimension of their varieties. Experimental results are provided to evaluate the complexity of solving SDP instances using our models through Gr\"obner bases techniques.

==> q7-SD-examples.tex <==
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\multicolumn{9}{c}{$q=7$}                                                   \\
 \hline 
$n$  & $k$  & $t$ & \# Lin Eqs & \# Quad Eqs & \# Vars & SR $d_{reg}$ & SD & \# Solutions \\ \hline
8  & 2  & 2  & 9        & 32        & 33    & 8       & 3  & 1            \\ \hline
8  & 4  & 1  & 7        & 32        & 33    & 10      & 3  & 6            \\ \hline
10 & 5  & 1  & 8        & 40        & 41    & 12      & 3  & 2            \\ \hline
16 & 2  & 6  & 17       & 64        & 65    & 13      & 3  & 1            \\ \hline
16 & 3  & 4  & 16       & 64        & 65    & 14      & 3  & 1            \\ \hline
16 & 4  & 4  & 15       & 64        & 65    & 14      & 3  & 1            \\ \hline
16 & 8  & 2  & 11       & 64        & 65    & 18      & 4  & 1            \\ \hline
16 & 8  & 1  & 11       & 64        & 65    & 18      & 4  & 1            \\ \hline
20 & 10 & 2  & 13       & 80        & 81    & 21      & 4  & 1           \\  \hline
\end{tabular}
\caption{This table gives information from experiments using Random $\mathbb{F}_7$-linear codes using the {\color{red} do we have a name?} modeling. 
 The value $\mathrm{sd}(S)$ is the solving degree of $S$, computed as the highest step degree achieved when directly computing the Gr\"obner basis of the system in MAGMA.
The values in the SD column give the highest step degree achieved when directly computing the Gr\"obner basis of the system in MAGMA. The SR $d_{reg}$ column gives the degree of regularity of a Semi-Regular system of equations with the associated number of linear equations, quadratic equations, and variables. }\label{Tab:q2-SolveDeg}
\end{table}
